Explaining Puzzle Solutions in Natural Language: An Exploratory Study on 6x6 Sudoku

The success of Large Language Models (LLMs) in human-AI collaborative decision-making hinges on their ability to provide trustworthy, gradual, and tailored explanations. Solving complex puzzles, such as Sudoku, offers a canonical example of this collaboration, where clear and customized explanations often hold greater importance than the final solution. In this study, we evaluate the performance of five LLMs in solving and explaining \sixsix{} Sudoku puzzles. While one LLM demonstrates limited success in solving puzzles, none can explain the solution process in a manner that reflects strategic reasoning or intuitive problem-solving. These findings underscore significant challenges that must be addressed before LLMs can become effective partners in human-AI collaborative decision-making.

==> interview_notes.tex <==
In the form of interview with a human solver

- Correct? — 
1. Does the explanation have any mistake in the reasoning process?

- Completeness/Helpfulness? —
1. Does it provide enough support for the explanation that it is given? It could be correct but the evidence provided might not be enough to suggest that solution (if not, explain why)
2. Does the explanation provide insight as to what thought process needs to happen to solve the problem? (If not, explain why)

- Selection/Focus? — 
1. Length of explanation (raw stats). 
2. What do the system/humans choose to focus on? 


— Solution (Done, quantify correctness)
— Given solution, can you explain this solution step by step. 

